EEND-DEMUX: End-to-End Neural Speaker Diarization via Demultiplexed Speaker Embeddings

In recent years, there have been studies to further improve the end-to-end neural speaker diarization (EEND) systems. This letter proposes the EEND-DEMUX model, a novel framework utilizing demultiplexed speaker embeddings. In this work, we focus on disentangling speaker-relevant information in the latent space and then transform each separated latent variable into its corresponding speech activity. EEND-DEMUX can directly obtain separated speaker embeddings through the demultiplexing operation in the inference phase without an external speaker diarization system, an embedding extractor, or a heuristic decoding technique. Furthermore, we employ a multi-head cross-attention mechanism to capture the correlation between mixture and separated speaker embeddings effectively. We formulate three loss functions based on matching, orthogonality, and sparsity constraints to learn robust demultiplexed speaker embeddings. The experimental results on the LibriMix dataset show consistently improved performance in both a fixed and flexible number of speakers scenarios.

==> algorithm.tex <==

\begin{algorithm}[t!]
    \caption{Training procedure of EEND-DEMUX}
    \label{algoritm}
    % \DontPrintSemicolon
    % \SetAlgoLined
    % \NoCaptionOfAlgo
    \scriptsize{
    % \footnotesize{
        % inputs
        % \KwIn{$T, \, S, \, \mathbf{X}, \, \mathbf{Y}, \, [\mathbf{X}_{1},\dots,\mathbf{X}_{S}], \,  \mathbf{p}, \, \mathcal{E}_{\theta}, \, \mathcal{D}_{\theta}, \, \mathcal{A}_{\theta}, \,$ and $\mathcal{S}_{\varphi}.$}
        \textsc{\textbf{Inputs:}} $T, \, S, \, \mathbf{X}, \, \mathbf{Y}, \, [\mathbf{X}_{1},\dots,\mathbf{X}_{S}], \,  \mathbf{p}, \, \mathcal{E}_{\theta}, \, \mathcal{D}_{\theta}, \, \mathcal{A}_{\theta}, \,$ and $\mathcal{S}_{\varphi}.$ \\
        % \KwOut{$\hat{\mathbf{Y}}^{\phi^{*}}$.}
        % \textsc{\textbf{Output:}} $\hat{\mathbf{Y}}^{\phi^{*}}$. \\

        \vspace{0.15cm}
        \For{$k= $ $ 1 $ to $ K$}{
            \vspace{0.05cm}
            $\textsc{Batch}_{k}
                \gets \{(\mathbf{X}^{i}, \mathbf{Y}^{i}, [\mathbf{X}_{1}^{i},\dots,\mathbf{X}_{S}^{i}])\}^{N}_{i=1}\sim$ \textsc{Training Dataset}\\
            
            \vspace{0.1cm}
            \For{$i= $ $ 1 $ to $ N$}{
                
                \vspace{0.1cm}
                $\mathbf{E}^{i} \,
                    \gets \mathcal{E}_{\theta}(\mathbf{X}^{i})$ \\

                \vspace{0.1cm}
                $[\hat{\mathbf{E}}^{i}_{1},\dots,\hat{\mathbf{E}}^{i}_{S}] 
                    \gets \mathcal{D}_{\theta}(\mathbf{E}^{i})$ \\

                \vspace{0.1cm}
                $[\hat{\mathbf{e}}^{i}_{\mu,1},\dots,\hat{\mathbf{e}}^{i}_{\mu,S}] 
                    \gets [\mathrm{TAP}(\mathbf{E}_{1}^{i}),\dots,\mathrm{TAP}(\mathbf{E}_{S}^{i})]$

                \vspace{0.1cm}
                $[\mathbf{a}^{i}_{1},\dots,\mathbf{a}^{i}_{S}] 
                    \gets \mathcal{A}_{\theta}(\hat{\mathbf{E}}^{i}_{\mu}, \mathbf{E}^{i})$

                \vspace{0.1cm}
                $\hat{\mathbf{Y}}^{i}
                    \gets \mathrm{sigmoid} ([\hat{\mathbf{E}}^{i}_{1} \odot \mathbf{a}^{i}_{1},\dots,\hat{\mathbf{E}}^{i}_{S} \odot \mathbf{a}^{i}_{S}])$

                \vspace{0.1cm}
                $\hat{\mathbf{p}}^{i} \> 
                    \gets \mathrm{sigmoid}(\mathrm{Linear}(\mathbf{A}^{i}))$

                \vspace{0.1cm}
                $[\mathbf{E}^{i}_{1},\dots,\mathbf{E}^{i}_{S}] 
                    \gets [\mathcal{S}_{\varphi}(\mathbf{X}_{1}^{i}),\dots,\mathcal{S}_{\varphi}(\mathbf{X}_{S}^{i})]$
                
                % the minimun permuted sequence
                \vspace{0.2cm}
                $\phi^{*} \>\,\,
                \gets {1 \over TS} \arg\min\nolimits_{\phi} \sum_{t} H(\mathbf{y}_{t}^{i\phi}, \hat{\mathbf{y}}_{t}^{i})$ \\
    
                % diarization loss
                \vspace{0.05cm}
                $\mathcal{L}_{\textnormal{diar}}^{i}
                \gets {1 \over TS} \sum_{t} H(\mathbf{y}_{t}^{i\phi^{*}}, \hat{\mathbf{y}}_{t}^{i})$ \\
    
                % existence loss
                \vspace{0.1cm}
                $\mathcal{L}_{\textnormal{ext}}^{i} \>
                \gets {1 \over S} H(\mathbf{p}^{i\phi^{*}}, \hat{\mathbf{p}}^{i})$ \\
    
                % distillation loss
                \vspace{0.1cm}
                $\mathcal{L}_{\textnormal{dis}}^{i} \>
                \gets {1 \over TS} \sum\nolimits_{t}\sum\nolimits_{s} || \mathbf{e}_{t,s}^{i\phi^*} - \hat{\mathbf{e}}_{t,s}^{i\phi^*} ||_{2} $ \\
    
                % orthogonality loss
                \vspace{0.1cm}
                $\mathcal{L}_{\textnormal{ort}}^{i} \>\,
                \gets {1 \over T {S \choose 2} } \sum_{t}\sum_{(i,j)} 1 - \underbrace{\langle \hat{\mathbf{e}}_{t,i}^{i\phi^*}, \hat{\mathbf{e}}_{\mu,i}^{i\phi^*}\rangle}_{\mathrm{pos}} + \gamma \underbrace{|\langle \hat{\mathbf{e}}_{t,i}^{i\phi^*}, \hat{\mathbf{e}}_{t,j}^{i\phi^*}\rangle|}_{\mathrm{neg}}$ \\
    
                % sparsity loss
                \vspace{-0.25cm}
                $\mathcal{L}_{\textnormal{spa}}^{i} \,
                \gets {1 \over TS} \sum\nolimits_{t}\sum\nolimits_{s} || \hat{\mathbf{e}}_{t,s}^{i} ||_{1}$ \\
    
                % total loss
                \vspace{0.1cm}
                $\mathcal{L}^{i} \>\>\,
                \gets \lambda_1 \mathcal{L}_{\textnormal{diar}}^{i}
                    + \lambda_2 \mathcal{L}_{\textnormal{ext}}^{i} 
                    + \lambda_3 \mathcal{L}_{\textnormal{dis}}^{i}
                    + \lambda_4 \mathcal{L}_{\textnormal{ort}}^{i}
                    + \lambda_5 \mathcal{L}_{\textnormal{spa}}^{i} $ 
            }

        % \vspace{0.05cm}
        $\theta_{k} \gets \theta_{k-1} - \eta_{k} {\partial \over \partial\theta}\left({1\over N}\sum_{i}{\mathcal{L}^{i}} \right)$ \\
        }
    }
\vspace{-0.1cm}
\end{algorithm}


==> table/legacy/libri23mix_min.tex <==
\begin{table}[t]
  \caption{Experimental results on combined Libri2Mix and Libri2Mix for \textit{min}.}
 
  \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  % \vspace{-4.0pt}
% \footnotesize{
  % \renewcommand{\tabcolsep}{1.80mm}
\begin{tabular}{l|ccccc}
\toprule
\multirow{2}{*}{Method} &  \multicolumn{5}{c}{Libri2Mix \& Libri3Mix}    \\
                        &  DER$\downarrow$    & FA$\downarrow$      & MI$\downarrow$      & CF$\downarrow$    & SCA$\uparrow$  \\

\midrule
TS-VAD [1]                                                                     & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

SA-EEND [1]                                                                    & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

EEND-EDA [2]                                                                   & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]                 & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$                                              & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF                 & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]                                                                       & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{spk}}$                                                   & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\
 
\midrule
EEND-MUX ($\mathcal{L}_{\text{diar}}$)                                             & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$                                                      & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                              & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                              & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$      & 2.49    & 1.93    & 1.91    & 1.35   & 0.00 \\

\bottomrule
\end{tabular}
  % }
  % \vspace{-10pt}
\end{table}

==> table/legacy/libri2mix_libri3mix_23conmined_min.tex <==
\begin{table*}[t]
  \caption{Experimental results on Libri2Mix or Libri3Mix for \textit{min} mode in terms of DER, FA, MI, and SCA(\%).}
   \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  % \vspace{-4.0pt}
\scriptsize{
  % \renewcommand{\tabcolsep}{1.80mm}
% \begin{tabular}{l|| c|ccc|c || c|ccc|c || c|ccc|c }
\begin{tabular}{l| cccc | cccc | ccccc }
\toprule
% \multirow{2}{*}{Method} &  \multicolumn{5}{c||}{Libri2Mix}    &  \multicolumn{5}{c||}{Libri3Mix}   & \multicolumn{5}{c}{Libri2Mix \& Libri3Mix}\\
%        &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$    &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$   &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$ \\
\multirow{2}{*}{Method} &  \multicolumn{4}{c|}{Libri2Mix \textit{min}}    &  \multicolumn{4}{c|}{Libri3Mix \textit{min}}   & \multicolumn{5}{c}{Libri2Mix \& Libri3Mix \textit{min}}\\
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$}       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$}       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$ \\



\midrule
SA-EEND [1]    & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35            & 2.49    & 1.93    & 1.91    & 1.35  & N/A  \\
TS-VAD [1]     & -       & -       & -       & -                  & -       & -       & -       & -               & 2.49    & -       & -       & -    & N/A \\
EEND-EDA [2]   & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -               & 2.49    & -       & -       & -     & 86.2 \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]          & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -               & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$                                             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF       & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{spk}}$                                                & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\


\midrule
EEND-MUX ($\mathcal{L}_{\text{diar}}$)                                                          & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$                                                                & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$      & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\



\bottomrule
\end{tabular}
  }
  % \vspace{-10pt}
\end{table*}

==> table/legacy/libri2mix_min.tex <==
\begin{table}[t]
  \caption{Experimental results on Libri2Mix or Libri3Mix for \textit{min} mode in terms of DER, FA, MI, and CF (\%).}
 
  \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  % \vspace{-4.0pt}
% \footnotesize{
  % \renewcommand{\tabcolsep}{1.50mm}
\begin{tabular}{l|c|cccc}
\toprule
\multirow{2}{*}{Method} &  \multicolumn{4}{c}{Libri2Mix-test \textit{min}}    \\
                                                  &  \multicolumn{1}{c}{DER ($\downarrow$)}    & FA ($\downarrow$)      & MI ($\downarrow$)      & CF ($\downarrow$)  \\
% \multirow{1}{*}{Method}   &  \multicolumn{1}{c|}{DER($\downarrow$)}    & FA($\downarrow$)      & MI($\downarrow$)      & CF($\downarrow$)  \\
\midrule
SA-EEND [1]                                                                                    & 2.49    & 1.93    & 1.91    & 1.35   \\

EEND-EDA [2]                                                                                   & 2.49    & 1.93    & 1.91    & 1.35   \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]                         & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$                                                            & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF                      & 2.49    & 1.93    & 1.91    & 1.35   \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]                            & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{spk}}$                                                               & 2.49    & 1.93    & 1.91    & 1.35   \\
 
\midrule
EEND-MUX ($\mathcal{L}_{\text{diar}}$)                                                         & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{dis}}$                                                               & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                                  & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                                  & 2.49    & 1.93    & 1.91    & 1.35   \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$     & 2.49    & 1.93    & 1.91    & 1.35   \\

\bottomrule
\end{tabular}
  % }
  % \vspace{-10pt}
\end{table}

==> table/legacy/libri3mix_min.tex <==
\begin{table}[t]
  \caption{Experimental results on Libri3Mix for \textit{min} mode in terms of DER, FA, MI, and SCA(\%).}
 
  \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  % \vspace{-4.0pt}
% \footnotesize{
  % \renewcommand{\tabcolsep}{1.80mm}
\begin{tabular}{l|cccc}
\toprule
Method                                                         &  DER$\downarrow$    & FA$\downarrow$      & MI$\downarrow$      & CF$\downarrow$     \\

\midrule
SA-EEND [1]                                                    & 2.49    & 1.93    & 1.91    & 1.35   \\

EEND-EDA [2]                                                   & 2.49    & 1.93    & 1.91    & 1.35   \\

\midrule
EEND-SS [3]                                                    & 2.49    & 1.93    & 1.91    & 1.35  \\

 - $\lambda_{1}=0$                                             & 2.49    & 1.93    & 1.91    & 1.35   \\

 + LMF                                                         & 2.49    & 1.93    & 1.91    & 1.35   \\

\midrule
EEND-MUX                                                       & 2.49    & 1.93    & 1.91    & 1.35   \\

 + $\lambda_{\text{dis}}$                                      & 2.49    & 1.93    & 1.91    & 1.35   \\

 + $\lambda_{\text{dis}}$, $\lambda_{\text{ort}}$              & 2.49    & 1.93    & 1.91    & 1.35   \\

 + $\lambda_{\text{dis}}$, $\lambda_{\text{spa}}$              & 2.49    & 1.93    & 1.91    & 1.35   \\

 + $\lambda_{\text{dis}}$, $\lambda_{\text{ort}}$, $\lambda_{\text{spa}}$     & 2.49    & 1.93    & 1.91    & 1.35   \\

\bottomrule
\end{tabular}
  % }
  % \vspace{-10pt}
\end{table}

==> table/legacy/table_all2_backup_20231006.tex <==
\begin{table*}[t]
  \caption{Experimental results in terms of DER, FA, MI, and SCA (\%). There are four evaluation protocols: Test sets of (1) Libri2Mix and (2) Libri3Mix of \textit{min} mode for \textit{fixed number of speakers} scenario. Test sets of (3-4) Libri2\&3Mix of \textit{min} and \textit{max} modes for \textit{flexible number of speakers} scenario. $\dagger$ indicates results by our re-implementation. }
   \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  \vspace{-4.0pt}
\scriptsize{
  \renewcommand{\tabcolsep}{1.40mm}
\begin{tabular}{l| cccc | cccc | ccccc | ccccc }
\toprule
\multirow{2}{*}{Method}    &  \multicolumn{4}{c|}{Libri2Mix \textit{min} (\textit{fixed})}    &  \multicolumn{4}{c|}{Libri3Mix \textit{min} (\textit{fixed})}   & \multicolumn{5}{c|}{Libri2\&3Mix \textit{min} (\textit{flexible})}   & \multicolumn{5}{c}{Libri2\&3Mix \textit{max} (\textit{flexible})}\\
% \multirow{3}{*}{Method}   
%     &  \multicolumn{8}{c|}{\it Fixed number of speakers}   &   \multicolumn{10}{c}{\it Flexible number of speakers} \\
%     &  \multicolumn{4}{c}{\it Libri2Mix \textit{min}}     & \multicolumn{4}{c|}{\it Libri3Mix \textit{min}}
    % &  \multicolumn{5}{c}{\it Libri2\&3Mix \textit{min}}  & \multicolumn{5}{c}{\it Libri2\&3Mix \textit{max}}\\
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$} 
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$} 
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & CF$\downarrow$  & \multicolumn{1}{c|}{SCA$\uparrow$} 
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & CF$\downarrow$   & SCA$\uparrow$ \\



\midrule
TS-VAD [1]               & -       & -       & -       & -                  & -       & -       & -       & -               & 5.30    & 2.83    & 2.32    & 0.15  & N/A           & 7.28    & 2.78    & 3.61    & 0.89  & N/A  \\
SA-EEND$^\dagger$ [1]    & 6.13    & 3.54    & 2.11    & 0.48               & 9.05    & 5.92    & 2.72    & 0.41            & 10.38   & 5.20    & 4.76    & 0.42  & N/A           & 11.42   & 6.21    & 4.50    & 0.71  & N/A  \\
EEND-EDA [2]             & 5.93    & -       & -       & -                  & 8.81    & -       & -       & -               & 10.16   & -       & -       & -     & 86.2          & -       & -       & -       & -     & -    \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]       & 5.26    & -       & -       & -             & 6.50    & -       & -       & -               & 8.79    & -       & -       & -     & 90.4             & -       & -       & -       & -     & -    \\

 + $\mathcal{L}_{\text{SI-SDR}}$                                             & 5.12    & -       & -       & -             & 6.26    & -       & -       & -               & 6.27    & -       & -       & -     & 97.9             & -       & -       & -       & -     & -    \\

 + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF       & 5.02    & -       & -       & -             & 6.00    & -       & -       & -               & 6.04    & -       & -       & -     & 98.2             & -       & -       & -       & -     & -    \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]          & -       & -       & -       & -             & -       & -       & -       & -               & 4.72    & 2.80    & 1.83    & 0.10  & -                & 6.49    & 2.81    & 3.04    & 0.65  & -    \\

 + $\mathcal{L}_{\text{spk}}$                                                & -       & -       & -       & -             & -       & -       & -       & -               & 4.48    & 2.60    & 1.79    & 0.08  & -                & 5.24    & 2.55    & 2.42    & 0.27  & -    \\


\midrule
EEND-DEMUX ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$)             & 4.67    & -       & -       & -             & -       & -       & -       & -              & -       & -       & -       & -       & -             & -       & -       & -       & -      & -    \\

 + $\mathcal{L}_{\text{dis}}$                                                & 4.18    & -       & -       & -             & -       & -       & -       & -              & -       & -       & -       & -       & -             & -       & -       & -       & -      & -    \\

 % + $\mathcal{L}_{\text{ort}}$                                                & 4.07    & -       & -       & -             & -       & -       & -       & -              & -       & -       & -       & -       & -             & -       & -       & -       & -      & -    \\

 + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                   & 4.02    & -       & -       & -             & -       & -       & -       & -              & -       & -       & -       & -       & -             & -       & -       & -       & -      & -    \\

 % + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                   & 4.22    & -       & -       & -             & -       & -       & -       & -              & -       & -       & -       & -       & -             & -       & -       & -       & -      & -    \\

 + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$  & \textbf{3.97}  & \textbf{2.69} & \textbf{1.12} & \textbf{0.10}      & \textbf{4.91} & \textbf{3.02} & \textbf{1.52} & \textbf{0.37}      & \textbf{4.38} & \textbf{2.55} & \textbf{1.78} & \textbf{0.05} & -             & -       & -       & -       & -      & -    \\



\bottomrule
\end{tabular}
  }
  % \vspace{-10pt}
\end{table*}

==> table/legacy/table_all_pre.tex <==
\begin{table*}[t]
  \caption{Experimental results on Libri2Mix or Libri3Mix for \textit{min} mode in terms of DER, FA, MI, and SCA(\%).}
   \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  \vspace{-4.0pt}
\scriptsize{
  \renewcommand{\tabcolsep}{1.00mm}
\begin{tabular}{l| cccc | cccc | ccccc }
\toprule
\multirow{2}{*}{Method} &  \multicolumn{4}{c|}{Libri2Mix \textit{min}}    &  \multicolumn{4}{c|}{Libri3Mix \textit{min}}   & \multicolumn{5}{c}{Libri2Mix \& Libri3Mix \textit{min}}\\
       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$}       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$}       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$ \\



\midrule
SA-EEND [1]    & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35            & 2.49    & 1.93    & 1.91    & 1.35  & N/A  \\
TS-VAD [1]     & -       & -       & -       & -                  & -       & -       & -       & -               & 2.49    & -       & -       & -    & N/A \\
EEND-EDA [2]   & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -               & 2.49    & -       & -       & -     & 86.2 \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]          & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -               & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$                                             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF       & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\

 \> + $\mathcal{L}_{\text{spk}}$                                                & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -                 & 2.49    & -       & -       & -     & 86.2 \\


\midrule
EEND-MUX ($\mathcal{L}_{\text{diar}}$)                                                          & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$                                                                & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\

 \> + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$      & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35           & 2.49    & 1.93    & 1.91    & 1.35  & 0.00 \\



\bottomrule
\end{tabular}
  }
  % \vspace{-10pt}
\end{table*}

==> table/legacy/table_fixed.tex <==
\begin{table}[t]
  \caption{Experimental results on Libri2Mix or Libri3Mix for \textit{min} mode in terms of DER, FA, MI, and SCA(\%).}
   \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  % \vspace{-4.0pt}
\scriptsize{
  \renewcommand{\tabcolsep}{1.1mm}
% \begin{tabular}{l|| c|ccc|c || c|ccc|c || c|ccc|c }
\begin{tabular}{l| cccc | cccc }
\toprule
% \multirow{2}{*}{Method} &  \multicolumn{5}{c||}{Libri2Mix}    &  \multicolumn{5}{c||}{Libri3Mix}   & \multicolumn{5}{c}{Libri2Mix \& Libri3Mix}\\
%        &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$    &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$   &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$}       & SCA$\uparrow$ \\
% \multirow{2}{*}{Method} &  \multicolumn{4}{c|}{Libri2Mix test \textit{min}}    &  \multicolumn{4}{c}{Libri3Mix test \textit{min}}  \\
%        &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$}       &  \multicolumn{1}{c}{DER$\downarrow$}    & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c}{CF$\downarrow$} \\
\multirow{2}{*}{Method} &  \multicolumn{4}{c|}{Libri2Mix \textit{min}}    &  \multicolumn{4}{c}{Libri3Mix \textit{min}}  \\
% \cmidrule{2-9}
       &  \multicolumn{1}{c}{DER$\downarrow$}    & \multicolumn{1}{c}{FA$\downarrow$}      & \multicolumn{1}{c}{MI$\downarrow$}      & \multicolumn{1}{c|}{CF$\downarrow$}       
       &  \multicolumn{1}{c}{DER$\downarrow$}    & \multicolumn{1}{c}{FA$\downarrow$}      & \multicolumn{1}{c}{MI$\downarrow$}      & \multicolumn{1}{c}{CF$\downarrow$} \\


\midrule
SA-EEND [1]    & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35    \\

EEND-EDA [2]   & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -       \\

\midrule
EEND-SS ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [3]          & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -       \\

 + $\mathcal{L}_{\text{SI-SDR}}$                                             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -         \\

 + $\mathcal{L}_{\text{SI-SDR}}$ + $\mathcal{L}_{\text{SI-SDR}}$ + LMF       & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -         \\

\midrule
USED ($\mathcal{L}_{\text{diar}}$ + $\mathcal{L}_{\text{ext}}$) [4]             & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -         \\

 + $\mathcal{L}_{\text{spk}}$                                                & 2.49    & -       & -       & -                  & 2.49    & -       & -       & -         \\


\midrule
EEND-MUX ($\mathcal{L}_{\text{diar}}$)                                                          & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35        \\

 + $\mathcal{L}_{\text{dis}}$                                                                & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35        \\

 + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35        \\

 + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{spa}}$                                   & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35        \\

 + $\mathcal{L}_{\text{dis}}$ + $\mathcal{L}_{\text{ort}}$ + $\mathcal{L}_{\text{spa}}$      & 2.49    & 1.93    & 1.91    & 1.35               & 2.49    & 1.93    & 1.91    & 1.35        \\

\bottomrule
\end{tabular}
  }
  % \vspace{-10pt}
\end{table}

==> table/table_all.tex <==
\begin{table*}[t]
  \caption{Experimental results in terms of DER, FA, and MI(\%). There are four evaluation protocols: Test sets of (1) Libri2Mix and (2) Libri3Mix of \textit{min} mode for \textit{fixed number of speakers} scenario. Test sets of (3-4) Libri2\&3Mix of \textit{min} and \textit{max} modes for \textit{flexible number of speakers} scenario. $\dagger$ indicates results by our re-implementation. }
   \centering
  % \setlength\tabcolsep{1.5pt}
  % \label{tab:main2}
  \vspace{-4.0pt}
% \scriptsize{
  % \renewcommand{\tabcolsep}{1.75mm}
\footnotesize{
  \renewcommand{\tabcolsep}{1.5mm}
\begin{tabular}{l| cccc | cccc | cccc | cccc }
\toprule
\multirow{2}{*}{\textbf{Method}}    &  \multicolumn{4}{c|}{\textbf{Libri2Mix} \textbf{\textit{min}} (\textbf{\textit{fixed}})}    &  \multicolumn{4}{c|}{\textbf{Libri3Mix} \textbf{\textit{min}} (\textbf{\textit{fixed}})}   & \multicolumn{4}{c|}{\textbf{Libri2\&3Mix} \textbf{\textit{min}} \textbf{(\textit{flexible}})}   & \multicolumn{4}{c}{\textbf{Libri2\&3Mix} \textbf{\textit{max}} \textbf{(\textit{flexible})}} \\
% \multirow{2}{*}{Method}    &  \multicolumn{4}{c|}{Libri2Mix \textit{min} (\textit{fixed})}    &  \multicolumn{4}{c|}{Libri3Mix \textit{min} (\textit{fixed})}   & \multicolumn{4}{c|}{Libri2\&3Mix \textit{min} (\textit{flexible})}   & \multicolumn{4}{c}{Libri2\&3Mix \textit{max} (\textit{flexible})} \\
        % &  \multicolumn{4}{c|}{\textbf{Libri2Mix} \textbf{\textit{min}} (\textbf{\textit{fixed}})}    &  \multicolumn{4}{c|}{\textbf{Libri3Mix} \textbf{\textit{min}} (\textbf{\textit{fixed}})}   & \multicolumn{4}{c|}{\textbf{Libri2\&3Mix} \textbf{\textit{min}} \textbf{(\textit{flexible}})}   & \multicolumn{4}{c}{\textbf{Libri2\&3Mix} \textbf{\textit{max}} \textbf{(\textit{flexible})}} \\
% \textbf{Method} 
        &  \multicolumn{1}{c}{DER$\downarrow$}   & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$} 
        &  \multicolumn{1}{c}{DER$\downarrow$}   & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$} 
        &  \multicolumn{1}{c}{DER$\downarrow$}   & FA$\downarrow$      & MI$\downarrow$      & \multicolumn{1}{c|}{CF$\downarrow$} 
        &  \multicolumn{1}{c}{DER$\downarrow$}   & FA$\downarrow$      & MI$\downarrow$      & CF$\downarrow$  \\

\midrule
TS-VAD [1]               & -       & -       & -       & -                  
                         & -       & -       & -       & -               
                         & 5.30    & 2.83    & 2.32    & 0.15           
                         & 7.28    & 2.78    & 3.61    & 0.89  \\
                         
SA-EEND$^\dagger$ [1]    & 6.13    & 3.54    & 2.11    & 0.48               
                         & 9.05    & 5.92    & 2.72    & 0.41            
                         & 10.38   & 5.20    & 4.76    & 0.42           
                         & 11.42   & 6.21    & 4.50    & 0.71  \\
                         
EEND-EDA [2]             & 5.93    & -       & -       & -                  
                         & 8.81    & -       & -       & -               
                         & 10.16   & -       & -       & -              
                         & -       & -       & -       & -     \\


\midrule
EEND-SS ($\mathcal{L}_{\textnormal{diar}}$ + $\mathcal{L}_{\textnormal{ext}}$) [3]       & 5.26          & -             & -             & -
                                                                             & 6.50          & -             & -             & -
                                                                             & 8.79          & -             & -             & -
                                                                             & -             & -             & -             & - \\


 + $\mathcal{L}_{\textnormal{SI-SDR}}$                                             & 5.12          & -             & -             & -             
                                                                             & 6.26          & -             & -             & -               
                                                                             & 6.27          & -             & -             & -                   
                                                                             & -             & -             & -             & - \\

 + $\mathcal{L}_{\textnormal{SI-SDR}}$ + $\mathcal{L}_{\textnormal{SI-SDR}}$ + LMF       & 5.02          & -             & -             & -
                                                                             & 6.00          & -             & -             & -               
                                                                             & 6.04          & -             & -             & -                   
                                                                             & -             & -             & -             & -     \\


\midrule
USED ($\mathcal{L}_{\textnormal{diar}}$ + $\mathcal{L}_{\textnormal{ext}}$) [4]          & -             & -             & -             & -             
                                                                             & -             & -             & -             & -               
                                                                             & 4.72          & 2.80          & 1.83          & 0.10                
                                                                             & 6.49          & 2.81          & 3.04          & 0.65  \\

 + $\mathcal{L}_{\mathrm{spk}}$                                                & -             & -             & -             & -             
                                                                             & -             & -             & -             & -               
                                                                             & 4.48          & 2.60          & 1.79          & \textbf{0.08}       
                                                                             & 5.24          & 2.55          & 2.42          & 0.27  \\


\midrule
EEND-DEMUX ($\mathcal{L}_{\textnormal{diar}}$ + $\mathcal{L}_{\textnormal{ext}}$)        & 4.67          & 2.83          & 1.52          & 0.32                
                                                                             & 5.64          & 3.51          & 1.68          & 0.45                    
                                                                             & 4.96          & 2.95          & 1.89          & 0.15             
                                                                             & 6.81          & 3.05          & 3.12          & 0.64    \\
                                                                             
 + $\mathcal{L}_{\textnormal{dis}}$                                                & 3.94          & 2.45          & 1.29          & 0.20                
                                                                             & 5.13          & 3.25          & 1.53          & \textbf{0.35}           
                                                                             & 4.55          & 2.61          & 1.82          & 0.12             
                                                                             & 5.19          & 2.50          & 2.44          & 0.25   \\
                                                                             
 + $\mathcal{L}_{\textnormal{dis}}$ + $\mathcal{L}_{\textnormal{ort}}$                   & 3.82          & 2.41          & \textbf{1.23} & 0.18       
                                                                             & 4.95          & 3.14          & 1.44          & 0.37                    
                                                                             & 4.43          & 2.57          & 1.77          & 0.09             
                                                                             & 5.12          & 2.49          & 2.41          & \textbf{0.22} \\
                                                                             
 + $\mathcal{L}_{\textnormal{dis}}$ + $\mathcal{L}_{\textnormal{ort}}$ + $\mathcal{L}_{\textnormal{spa}}$          & \textbf{3.79} & \textbf{2.38} & 1.25          & \textbf{0.16}      
                                                                                                 & \textbf{4.91} & \textbf{3.12} & \textbf{1.42} & 0.37      
                                                                                                 & \textbf{4.39} & \textbf{2.53} & \textbf{1.76} & 0.10       
                                                                                                 & \textbf{5.08} & \textbf{2.46} & \textbf{2.38} & 0.24           \\
\bottomrule
\end{tabular}
  }
  % \vspace{-10pt}
\end{table*}
